Media-Based Modulation for Next-Generation Wireless: A Survey and Some New Developments

The idea of media-based modulation (MBM) is to embed information in the channel states via intentional perturbations of the transmission media. This article covers a broad range of topics regarding MBM, expanding on its benefits and reviewing relevant challenges, alluding to potential future research directions. The article starts by arguing how MBM differs from a source-based modulation; we highlight the key shortcomings in a legacy multiple-input multiple-output (MIMO) system that MBM sets out to address, including the issue of deep fades and MIMO diversity-multiplexing trade-off. The article further explains how MBM works in harmony with other index modulations and improves upon them by providing similar advantages with a more compact transmitter. Numerical results (simulation and analytical) are provided to support the claims on the discussed benefits. The highlights of numerical results include: 1) outage comparison with legacy MIMO systems; 2) comparisons with other state-of-the-art modulation schemes such as generalized spatial modulation; and 3) performance example of sending 32 bits of information in a single transmission with an excellent symbol error rate of $\mathsf{SER} \simeq 10^{-5}$ at \say{energy per bit to noise power spectral density ratio} of $\mathsf{E_b/N_0} \simeq -3.5$ dB. The article continues with methods to address the issues of receiver training and decoding for large constellation sets. A number of other research questions, such as pulse shaping to limit spectral growth due to the time-varying nature of MBM and the effect of forward error correcting codes on MBM diversity order are discussed. Finally, an RF transceiver structure is presented to generate independent propagation paths for embedding information. Fabrication and testing of the transceiver structure show close agreement between simulation and measurement.

==> RFfigs.tex <==
\begin{figure}[]
\centering
\includegraphics[width=0.95\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/Fig_XXXVII.jpg}
\caption{$S_{11}$ of the TX antenna with flat caps (simulation results).}
\label{fig:S11_flat}
\end{figure}

\begin{table*}
\begin{center}
\caption{Antenna radiation parameters at 5.8535 GHz  for flat caps (case 1) and for caps with optimized curvatures (case 2). Maximum gain values are computed over a partial spherical far-field surface with $\theta$ deviating ±20\degree from the horizontal plane. Accepted power accounts only for the impact of $S_{11}$. Radiated Power accounts for the impact of $S_{11}$, as well as for the waste of energy in antenna structure. Radiated Power is computed by integrating the energy density, i.e, the Poynting vector, over a sphere (at far-field) surrounding the entire antenna structure. Efficiency is defined as the ratio: Radiated Power/Incident Power.}
\begin{tabularx}{0.9\textwidth} { 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X  | }
  \hline
  Quantity & case 1 & case 2 \\
  \hline
   Incident Power & 1 W & 1W \\
  \hline
    Accepted Power & 851.6 mW & 957.74 mW \\
  \hline
  Radiated Power & 820.9 mW  & 903.28 m\\
  \hline
  Efficiency & 82.1\% & 90.3\% \\ \hline
    Peak Realized Gain & 2.3468 & 5.9575 \\
  \hline
\end{tabularx}
\end{center}
\end{table*}

\begin{table*}
\begin{center}
\caption{TX antenna dimensions (reported in mm)}
\begin{tabularx}{0.9\textwidth} { 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X  | }
  \hline
  w0 & w1 & w2 & w3 & w4 & w5 & h1 & h2 & h3 & h4 & h5 & w6 & w7 & w8 & h6 & h7 & h8\\ 
  \hline
  1.008 & 0.5 & 1.25 & 0.7 & 2.5 & 3 & 9 & 13 & 16 & 20 & 30 & 1.5 & 4 & 10 & 5 & 6.5 & 9\\ 
  \hline
\end{tabularx}
\label{tab:tx_antenna_dimensions}
\end{center}
\end{table*}

\begin{figure}[]
\begin{subfigure}{\textwidth}
  \centerline{\hspace*{-9.5cm}\includegraphics[width=0.5\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/Fig30_a.jpg}}
\end{subfigure}
\\
\begin{subfigure}{\textwidth}
\vspace{1.5cm}
   \centerline{\hspace*{-9.5cm}\includegraphics[width=0.5\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/Fig30_b.jpg}}
\end{subfigure}
\caption{Simulation results for square patch length of 4mm for two states of ON and OFF, a) reflection, b) transmission.}
\label{fig:simulation_result}
\end{figure}

\begin{table*}
\begin{center}
\caption{RX antenna dimensions}
\begin{tabularx}{0.9\textwidth} { 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X  | }
  \hline
  w0 & w1 & w2 & w3 & w4 & h1 & h2 & h3 & h4 & h5 & h6\\ 
  \hline
  0.5mm & 0.75mm & 1.5mm & 6.5mm & 10.5mm & 3.3mm & 7.3mm & 11.3mm & 12.05mm & 16.8mm & 21.55mm\\ 
  \hline
\end{tabularx}
\label{tab:rx_antenna_dimensions}
\end{center}
\end{table*}

\begin{figure}[]
 \centerline{\includegraphics[width=1\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/Fig32.jpg}}
\caption{RX antenna input matching.}
\label{fig:input_matching}
\end{figure}

\begin{table*}
\begin{center}
\caption{Different walls' states selected for simulation of $S_{11}$ in Fig.~\ref{fig:tx_input_matching}. Note that, even though each of the three RF building blocks forming a wall can be switched independently, in simulation results of Fig.~\ref{fig:tx_input_matching}, all switches on any of the walls $1$ to $12$ have the same state (i.e., all are ON for value 1, or all are off for value zero).}
\begin{tabularx}{0.9\textwidth} { 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X  | }
  \hline
  State No & Sw1 & Sw2 & Sw3 & Sw4 & Sw5 & Sw6 & Sw7 & Sw8 & Sw9 & Sw10 & Sw11 & Sw12\\ 
  \hline
  1 & 0 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 0 & 1 & 1 & 0\\ 
  \hline
  2	& 1	& 0	& 0	& 1	& 1	& 1	& 0	& 0 & 0 & 1 & 1 & 0 \\
  \hline
  3	& 1	& 1 & 1 & 0 & 0 & 1 & 1 & 0 & 1 & 1 & 1 & 0 \\
  \hline
  4	&1	&1	&1	&0	&0	&0	&1	&1	&1	&0	&0	&0 \\
  \hline
  5	&1	&0	&0	&0	&0	&1	&1	&0	&0	&1	&1	&1 \\
  \hline
  6	&1	&1	&1	&0	&0	&0	&0	&0	&0	&1	&1	&1 \\
  \hline
  7	&1	&0	&1	&0	&1	&0	&1	&0	&1	&1	&0	&1 \\
  \hline
\end{tabularx}
\end{center}
\end{table*}


\begin{figure*}[]
\centering
\includegraphics[width=0.8\linewidth, trim={0, 0cm, 0, 1cm}]{./fig_rf/S11-sim}
\caption{$S_{11}$ of the TX antenna, with optimized caps, for 7 different walls states mentioned in Table 2 (emulation results).}
\label{tx_input_matching}
\end{figure*}


\begin{figure}[tb]
    \centerline{\includegraphics[scale = 0.36]{./fig_rf/building-block2.png}}
	\caption{(a) An RF building block with RF switches being open (approximated as "open circuit''). (b) An RF building block with RF switches being closed (approximated as "short circuit''). (c)  Periodic repetition of the RF building block in (b), i.e., with switches being closed.}
	\label{Fig:build}
\end{figure}

\begin{figure}[htbp]
    \centerline{\includegraphics[scale = 0.6]{./fig_rf/RX-pattern.jpg}}
	\caption{Pattern of a receive antenna in the presence of the entire antenna structure. }
	\label{RX-pattern}
\end{figure}


\begin{figure}[tb]
    \centerline{\includegraphics[scale = 0.31]{./fig_rf/TX-pattern-all.jpg}}
	\caption{Pattern of the transmit antenna in the absence of the top and bottom metallic closures. (b) Transmit antenna in the presence of the top and bottom metallic closures. (c) Pattern of the transmit antenna in the presence of the top and bottom metallic closures. }
	\label{TX-all}
\end{figure}


\begin{figure}[!ht]
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{./fig_rf/Fig22_a_bmp.pdf}
  \caption{}
  \label{fig:sfig1}
\end{subfigure}%
\\
\begin{subfigure}{.45\textwidth}
   \centering
   \includegraphics[width=1.06\linewidth]{./fig_rf/Fig22_b_bmp.pdf}
     \caption{}
  \label{fig:sfig2}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
   \centering
   \vspace*{0.3cm} \hspace*{1.2cm}\includegraphics[width=0.93\linewidth]{./fig_rf/Numbering.jpg}
     \caption{}
  \label{fig:sfig3}
\end{subfigure}
\caption{The multi-pattern structure, a) view from the top, b) view from the bottom, c) view from the inside (including the indexing of switches used as labels in Table~\ref{??}.}
\label{fig:multi-pattern_structure}
\end{figure}
\begin{figure}[!ht]
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{./fig_rf/Fig22_d.jpg}
  \caption{}
\end{subfigure}%
\\
\begin{subfigure}{.45\textwidth}
    \centering
    \vspace*{0.1cm}\includegraphics[width=1\linewidth]{./fig_rf/Fig22_e.jpg}
    \caption{}
\end{subfigure}
\caption{The multi-pattern structure, a) top view, b) upside down. There are twelve walls, each with 3 columns of switchable parasitic elements and one receive antenna in each wall. }
\label{fig:multi-pattern_structure2}
\end{figure}

\begin{figure}[!ht]
\begin{subfigure}{.45\textwidth}
  \centerline{\vspace*{-0.7cm}\includegraphics[width=1\linewidth]{./fig_rf/Fig24_a_bmp.pdf}}
  \caption{}
\end{subfigure}%
\\
\begin{subfigure}{.45\textwidth}
   \centerline{\includegraphics[width=1\linewidth]{./fig_rf/Fig24_b_2_bmp.pdf}}
     \caption{}
\end{subfigure}
\caption{Top hat: a) top view, b) bottom view.}
\label{top_hat}
\end{figure}

\begin{figure}[!ht]
\begin{subfigure}{.45\textwidth}
  \centerline{\includegraphics[width=1\linewidth]{./fig_rf/Fig25_a_2_bmp.pdf}}
  \caption{}
\end{subfigure}%
\\
\begin{subfigure}{.45\textwidth}
   \centerline{\vspace*{-0.5cm}\includegraphics[width=1.1\linewidth]{./fig_rf/Fig25_b_bmp.pdf}}
     \caption{}
\end{subfigure}
\caption{Bottom hat: a) top view, b) bottom view.}
\label{bottom_hat}
\end{figure}

\begin{figure}[!h]
\begin{subfigure}{.45\textwidth}
  \centerline{\includegraphics[width=1\linewidth]{./fig_rf/Fig30_aa.pdf}}
  \caption{}
\end{subfigure}%
\\
\begin{subfigure}{.45\textwidth}
   \centerline{\includegraphics[width=1\linewidth]{./fig_rf/Fig30_bb.pdf}}
     \caption{}
\end{subfigure}
\caption{TX antenna, a) front view, b) back view.}
\label{fig:tx_antenna}
\end{figure}

\begin{figure}[b]
\centering 
\includegraphics[width=.9\linewidth]{./fig_rf/Fig_Walls_Structure.jpg}
\caption{Structure of the walls. Left structure shows each column of 13 switches (PIN diodes) that are controlled independently. The structure on the right shows one of 12 receiver antennas.}
\label{fig:wall_structure}
\end{figure}

\begin{figure}[]
\begin{subfigure}{.5\textwidth}
  \centerline{\includegraphics[width=1\linewidth]{./fig_rf/Fig13_a.pdf}}
  \caption{}
\end{subfigure}%
\\
\begin{subfigure}{.5\textwidth}
   \centerline{\includegraphics[width=1\linewidth]{./fig_rf/Fig13_b.pdf}}
     \caption{}
\end{subfigure}
\caption{Control board PCB, a) top layer, b) bottom layer.}
\label{fig:control_board}
\end{figure}

%
%\begin{figure}[t]
%\centerline{\includegraphics[width=1.\linewidth]{./fig_rf/S11-RX}}
%\caption{$S_{11}$ of the RX antenna (measurement result).}
%\label{fig:S11_RX}
%\end{figure}

\begin{figure*}[t]
\centerline{\includegraphics[width=1.\linewidth]{./fig_rf/S11}}
\caption{$S_{11}$ of the TX antenna (with optimized caps) for some configurations of ON/OFF switches (measurement results).}
\label{fig:S11_measure}
\end{figure*}



==> rf_implementation_v0.tex <==
\section{Radio Frequency Implementation} \label{RF-sec}

Reference \cite{lmimo_mbm} (also see~\cite{7511273}) reports an MBM antenna unit operating at 5.8 GHz. Fig.  \ref{single_rf_chain} shows an LMBM structure relying on the corresponding antenna. The RF structure in \cite{lmimo_mbm} enjoys low hardware complexity, as it incorporates a single transmit chain, where an RF divider is used to feed multiple transmit antennas. The RF phase shifters in Fig. \ref{single_rf_chain} allow sending additional SBM data. For example, one can select 0\degree, 90\degree, 180\degree, and 270\degree~phase shifts according to two additional bits of SBM data (per transmit unit). Reference \cite{lmimo_mbm} discusses techniques, including the use of RF phase shifters in  Fig.~\ref{single_rf_chain}, to facilitate receiver training. The same techniques apply to the new antenna structure presented in the current article. Readers are referred to~\cite{Tech-rep1}  for examples of antenna patterns and realizations of MBM constellations corresponding to indoor and outdoor propagation environments (also see~\cite{isit2014} for the latter). Simulations are performed using ANSYS high-frequency structural simulator (ANSYS HFSS\footnote{\href{www.ansys.com/products/electronics/ansys-hfss}{www.ansys.com/products/electronics/ansys-hfss}}) to obtain antenna patterns, which are then imported to the ray tracing software (Remcom Wireless Insite\footnote{\href{https://www.remcom.com/wireless-insite-em-propagation-software}{https://www.remcom.com/wireless-insite-em-propagation-software}}) to obtain the constellation points.  
%It is observed that the constellation structure enjoys the desired randomness in all three propagation environments (indoor, outdoor, and line-of-sight).

\begin{figure}
\hspace{0 cm}
\vspace{-0.2cm}
%\includegraphics[width=0.95\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/TX2.jpg}
\includegraphics[width=\columnwidth]{./fig_rf/TX2.jpg}
\caption{Overall structure of a transmitter with multiple transmit antennas.}
\label{single_rf_chain}
\end{figure}

Antenna structure reported in \cite{Tech-rep1}, although tested for functionality (see \cite{new-ak1}, \cite{new-ak2}), suffers from the following shortcomings: 
\begin{enumerate}
    \item The top and bottom of the antenna's cylindrical shape are left open. Consequently, part of the energy of the radio frequency wave leaves the transmitter through the top/bottom openings. This, in turn, reduces the antenna gain in the horizontal plane.  
    \item It lacks any receive (RX) antenna. 
\end{enumerate}
Fig. \ref{fig:multi-pattern_structure} and \ref{fig:multi-pattern_structure2} show the new antenna structure designed to address the above shortcomings. The new structure includes: 1) metallic reflectors closing the top and the bottom; and 2) each wall includes a receive (RX) antenna. 

\begin{figure}[!ht]
\begin{subfigure}{.45\textwidth}
  \centering
  %\includegraphics[width=1.06\linewidth]{./fig_rf/comb1.jpg}
   \includegraphics[width =\columnwidth]{./fig_rf/comb1.jpg}
  \caption{}
\end{subfigure}%
\\
\begin{subfigure}{.48\textwidth}
    \centering
    \vspace*{0.1cm}\includegraphics[width=1\columnwidth]{./fig_rf/sel2.jpg}
    \caption{}
\end{subfigure}
\caption{Antenna structure: (a) some components, plus a partially assembled antenna structure, (b) fully assembled antenna structure. There are twelve walls, each with three building block columns  of switchable parasitic elements and one receive antenna in each wall. Building block columns, in total 36, are controlled independently.}
\label{fig:multi-pattern_structure}
\end{figure}

\begin{figure}
\centering
%\includegraphics[width=0.95\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/Fig_XXXVII.jpg}
\includegraphics[width=0.75\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/setz.jpg}
\caption{Antenna structure: (a) view from the top, (b) view from the bottom, (c) view from the inside - including indexing of walls used in Table~\ref{Tabclw2}.}
\label{fig:multi-pattern_structure2}
\end{figure}

\begin{comment}
\begin{figure}[!ht]
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{./fig_rf/Fig22_a_bmp.pdf}
  \caption{}
  \label{fig:sfig1}
\end{subfigure}%
\\
\begin{subfigure}{.45\textwidth}
   \centering
   \includegraphics[width=1.06\linewidth]{./fig_rf/Fig22_b_bmp.pdf}
     \caption{}
  \label{fig:sfig2}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
   \centering
   \vspace*{0.3cm} \hspace*{1.2cm}\includegraphics[width=0.93\linewidth]{./fig_rf/Numbering.jpg}
     \caption{}
  \label{fig:sfig3}
\end{subfigure}
\caption{New antenna structure: (a) view from the top, (b) view from the bottom, (c) view from the inside - including indexing of walls used in Table~\ref{Tabclw2}.}
\label{fig:multi-pattern_structure2}
\end{figure}

\begin{figure}[!ht]
\begin{subfigure}{.45\textwidth}
  \centerline{\vspace*{-1cm}\includegraphics[width=1\linewidth]{./fig_rf/Fig24_a_bmp.pdf}}
  \caption{}
\end{subfigure}%
\\
\begin{subfigure}{.45\textwidth}
   \centerline{\includegraphics[width=1\linewidth]{./fig_rf/Fig24_b_2_bmp.pdf}}
     \caption{}
\end{subfigure}
\caption{Top hat: (a) top view, (b) bottom view.}
\label{top_hat}
\end{figure}

\begin{figure}[!ht]
\begin{subfigure}{.45\textwidth}
  \centerline{\vspace*{-0.3cm}\includegraphics[width=1\linewidth]{./fig_rf/Fig25_a_2_bmp.pdf}}
  \caption{}
\end{subfigure}%
\\
\begin{subfigure}{.45\textwidth}
   \centerline{\vspace*{-0.5cm}\includegraphics[width=1.1\linewidth]{./fig_rf/Fig25_b_bmp.pdf}}
     \caption{}
\end{subfigure}
\caption{Bottom hat: (a) top view, (b) bottom view.}
\label{bottom_hat}
\end{figure}


\begin{figure}[b]
\centering 
\includegraphics[width=0.9\linewidth]{./fig_rf/sel1.jpg}
\caption{Structure of the walls. Left structure shows each building block column  of 13 switches (PIN diodes) that are controlled independently. The structure on the right shows one of 12 receiver antennas.}
\label{fig:wall_structure}
\end{figure}
\end{comment}


\begin{figure}[tb]
    \centerline{\includegraphics[scale = 0.7]{./fig_rf/TX-pattern-all.jpg}}
	\caption{Pattern of the transmit antenna: (a) in the absence of the top and bottom metallic closures, (b) in the presence of the top and bottom metallic closures shown in (c). }
	\label{TX-all}
\end{figure}


In this new design, each wall includes three building-block columns of RF patches where RF switches corresponding to different columns can be controlled (turned on/off) independently.      
Transmit (TX) antenna, which is located at the center of this structure (fixed to the bottom cap) - see Fig.~\ref{TX-all}(c), is designed to generate an Omni-directional pattern (in the absence of the other parts) - see Fig.~\ref{TX-all}(a). The reason for an Omni-directional TX pattern is explained next. 
Noting the symmetry of the antenna walls  along the spherical angle $\phi$ (i.e., in the X-Y plane), it is desirable to have a transmit  pattern with a similar spherical symmetry. Such a spherical symmetry guarantees that each of the 12 RF walls is exposed to (approximately) the same amount of RF energy. Consequently, when switched on and off, each RF wall has (approximately) the same impact on the outgoing RF signal. Accordingly, the transmitter can provide coverage for any receiver located at an angle of $\phi\in[0,360\degree]$ (with respect to the transmit unit). 
The two metallic reflectors/closures, called metallic caps hereafter, are responsible for constraining the radiation in the horizontal directions - compare the TX pattern in Fig. \ref{TX-all}(a) vs. the one in Fig. \ref{TX-all}(b). 
%The top and bottom ribs in each wall PCB pass through respective slots on top and bottom caps, holding the entire structure together.  
%We have used a 100mm long Polyamide Hex spacer at each corner, and have fixed the entire structure using Nylon screws and nuts. 
There are three building block columns on each wall, each with thirteen patches, one large metallic rectangular patch on the interior, and a single RX antenna on the exterior. The thirteen small patches in each building block column  are connected to each other using RF switches (PIN diodes). When the switches on a given building block column are on (low impedance connection), the corresponding patches form a connected metallic strip that reflects the incident wave back to the interior of the antenna structure. If the switches are off, the incident wave results in an RF signal propagating to the outside of the antenna structure (i.e., the corresponding building block column acts as if it were transparent to the incident wave). To optimize the geometry of each wall, one needs to devise a computational method that can find an initial approximate solution (with acceptable performance) in a reasonable time. Then, one can include the initial solution obtained in this manner within the entire antenna structure and rely on HFSS to tune (optimize) the underlying dimensions. The basic building block structure is repeated periodically to achieve this goal, forming a plane extending to infinity. Fig. \ref{Fig:build}(a) and \ref{Fig:build}(b) show a single building block column in off and on states, respectively, and Fig.   \ref{Fig:build}(c) shows the periodic extension of a single building block column in the on state. 
The periodic extension in Fig.~\ref{Fig:build} provides an acceptable starting point for subsequent HFSS optimization. This is due to the fact that, in the actual antenna structure, columns are placed around a circle mimicking an infinite extension along the X axis in Fig.~\ref{Fig:build}(c), while reflections in the top and bottom metallic caps mimic an infinite extension along the Y axis. Relying on HFSS, a plane wave (with a vertical polarization), propagating along the $-z$ axis, is incident on the periodically extended structure in Fig.\ref{Fig:build}(c), then the energy of the wave propagating to the opposite side is measured and used to compute $S_{12}$ and $S_{11}$ (indices 1 and 2 refer to the two sides of the periodically extended surface). In the RF domain, this is achieved by relying on the concept of Floquet ports\footnote{https://courses.ansys.com/index.php/courses/ansys-hfss-floquet-port.}. Upon including the resulting initial design within the rest of the antenna structure, the dimensions of the basic patch element are further optimized (using HFSS) to achieve the curves shown in Fig.~\ref{simulation_result}(a) and (b) for $S_{12}$ and $S_{11}$, respectively.  The large patch on each wall acts as the RX antenna ground plane.    

\begin{figure}[tb]
    \centerline{\includegraphics[scale = 0.36]{./fig_rf/building-block.jpg}}
	\caption{(a) An RF building block with RF switches being open (approximated as ``open circuit''). (b) An RF building block with RF switches being closed (approximated as ``short circuit''). (c)  Periodic repetition of the RF building block in (b), i.e., with switches being closed.}
	\label{Fig:build}
\end{figure}

\begin{figure}[]
\begin{subfigure}{\textwidth}
    \centerline{\hspace*{-9.5cm}\includegraphics[width=0.5\linewidth]{./fig_rf/Fig30_b.jpg}}
    %\centerline{\hspace*{-9.5cm}\includegraphics[width=0.5\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/square_patch_S12.pdf}}
\end{subfigure}
\\
\begin{subfigure}{\textwidth}
\vspace{0cm}
   \centerline{\hspace*{-9.5cm}\includegraphics[width=0.5\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/Fig30_a.jpg}}
   %\centerline{\hspace*{-9cm}\includegraphics[width=0.45\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/square_patch_S11.pdf}}
\end{subfigure}
\caption{Simulation results for the rectangular patch in two states of on and off: (a) transmission and (b) reflection. In these simulations, dimensions of the basic patch (optimized relying on periodic extension) is 4\,mm by 5\,mm.  Upon integrating this initial patch geometry within the rest of the antenna structure, and further tuning, the final patch dimensions are set at 5.6\,mm by 6\,mm. }
\label{simulation_result}
\end{figure}


%\begin{figure}[]
 %\centerline{\includegraphics[width=1\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/Fig32.jpg}}
 %\centerline{\includegraphics[width=1\linewidth, trim={0, 0cm, 0, %0cm}]{./fig_rf/RX1.jpg}}

 %\caption{RX antenna input matching (a) HFSS simulation).}
%\label{fig:input_matching}
%\end{figure}

\subsection{Top and Bottom Caps: Detailed Derivations}

In a preliminary design, we used two flat metallic caps to close the top and the bottom of the antenna structure (see Fig.~\ref{flat}). It was observed that the impedance matching of the TX antenna could not be improved beyond -10 dB - see Fig.~\ref{fig:S11_flat} for the corresponding $S_{11}$ graphs.
To improve the impedance matching, a cap structure was designed to guide the incident RF wave (see Fig.~\ref{fig:multi-pattern_structure}, \ref{fig:multi-pattern_structure2} and ~\ref{TX-all}). Another benefit of these caps would be higher efficiency  (see Table~\ref{TabIII}) and a pattern focused around the horizontal plane (see Fig.~\ref{TX-all}). Fig.~\ref{tx_input_matchingm}, obtained through measurement, confirms the claim that (using the curved caps) the $S_{11}$ parameter is rather insensitive to the switching pattern, and values for different switching patterns remain at an acceptable level. 

\begin{figure}[]
\centering
%\includegraphics[width=0.95\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/Fig_XXXVII.jpg}
\includegraphics[width=0.7\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/flat2}
\caption{Antenna with flat caps.}
\label{flat}
\end{figure}

\begin{figure}[]
\centering
%\includegraphics[width=0.95\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/Fig_XXXVII.jpg}
\hspace{-0.5cm}\includegraphics[width=0.9\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/s11_flat.pdf}

\caption{$S_{11}$ of the TX antenna with flat caps (HFSS simulation).}
\label{fig:S11_flat}
\end{figure}

\begin{figure}[tbp]
%\centerline{\includegraphics[width=.9\linewidth]{./fig_rf/Fig2.pdf}}
\centerline{\includegraphics[scale=0.23]{./fig_rf/image-3.png}}
\caption{The curvature of the proposed cap.}
\label{fig:curvature}
\end{figure}

%In the initial design, we used two flat metallic caps on top and bottom of the structure, but it resulted that the radiation efficiency fell around 60\% and also make the TX antenna matching very difficult and sensitive to the state of PIN diodes on walls, so we decided to design the top and bottom caps such that they reflect the rays initiating from the origin parallel to the horizontal plane (Fig. \ref{fig:curvature}). The curvature of the interior surface of the proposed cap is shown in Fig. \ref{fig:curvature}.

The top and bottom caps are designed to reflect a ray initiating from the origin such that it propagates parallel to the horizontal axis. The curvature of a cut in the interior surface of the proposed cap is shown in Fig. \ref{fig:curvature}. Let us assume a radiating point source is located at the origin, i.e.,  $(0, 0)$. The cap surface, which is obtained by rotating the function of $y=f(x)$ around the $y$-axis, should reflect a ray originating from such a point source parallel to the $x$-axis. Referring to Fig.~\ref{fig:curvature}, this means 

\begin{IEEEeqnarray}{c}
\alpha + 2 \theta = \pi.
\label{eq:rf1}
\end{IEEEeqnarray}
We also have
\begin{IEEEeqnarray}{c}
\alpha = \beta  + \frac{\pi}{2} - \theta.
\label{eq:rf2}
\end{IEEEeqnarray}
By eliminating $\theta$ in \eqref{eq:rf1} and \eqref{eq:rf2}, we obtain 
\begin{IEEEeqnarray}{c}
\alpha=2\beta.	
\label{eq:rf4}
\end{IEEEeqnarray}
The dashed line in Fig.~\ref{fig:curvature} intersecting with the $x$ axis is tangent to the curve $y=f(x)$. Therefore, 
\begin{IEEEeqnarray}{c}
f^{\prime}(x) = y^{\prime} = \tan(\beta).
\label{eq:rf3}
\end{IEEEeqnarray}
By substituting \eqref{eq:rf4} in \eqref{eq:rf3}, and noting $\tan{\left(\alpha\right)}={y}/{x}$,
%\begin{equation}
%\tan{\left(\alpha\right)}={y}/{x},
%\end{equation} 
it follows that 
\begin{IEEEeqnarray}{c}
{\tan}^{-1}\left(\frac{y}{x}\right) = 2{\tan}^{-1}\left(y^\prime\right). 
\label{eq:tan_inv}
\end{IEEEeqnarray}
Taking $\tan$ of the two sides of \eqref{eq:tan_inv} and using the identity $\tan(2a) = 2\tan(a)/(1-\tan^2(a))$, we obtain
% Ehsan, is it the "above equation"? -> referenced it with a number
\begin{IEEEeqnarray}{LL}
\frac{y}{x} &= \tan {\left(2{\tan}^{-1}\left( y^\prime \right)\right)} \\
 &= \frac{y^{\prime}}{1-{y^{\prime}}^2}.
\label{eq:rf5}
\end{IEEEeqnarray}
Equation \eqref{eq:rf5} is a quadratic equation of the form
\begin{IEEEeqnarray}{c}
{y^{\prime}}^2+2\frac{x}{y}y^\prime-1 = 0
\label{eq:quadratic_diff}
\end{IEEEeqnarray}
in $y^{\prime}$. Referring to Fig.~\ref{fig:curvature}, since $y>0$ and $y^{\prime}>0$, the quadratic equation \eqref{eq:quadratic_diff} has a single valid solution of the form
\begin{IEEEeqnarray}{c}
\frac{y^\prime}{y}=\frac{1}{x+\sqrt{x^2+y^2}}.	
\end{IEEEeqnarray}
To solve the above differential equation, we perform some manipulations as follows:
\begin{IEEEeqnarray}{c}
x\frac{y^\prime}{y}+\frac{y^\prime}{y}\sqrt{x^2+y^2}-1=0.
\end{IEEEeqnarray}
Since $y>0$, we have
\begin{IEEEeqnarray}{c}
\frac{x\frac{y^\prime}{y}+\frac{y^\prime}{y}\sqrt{x^2+y^2}-1}{\sqrt{x^2+y^2}}\times\frac{-x+\sqrt{x^2+y^2}}{-x+\sqrt{x^2+y^2}}=0.
\label{eq:rf9}
\end{IEEEeqnarray}
Let us define $U:=-x+\sqrt{x^2+y^2}$ and ${U^\prime} := \mathrm{d}U/ \mathrm{d}x$. Then, \eqref{eq:rf9} simplifies to
\begin{IEEEeqnarray}{c}
\frac{U^\prime}{U}=0\rightarrow\ln{\left(U\right)}=c,
\label{Eq-ak2}
\end{IEEEeqnarray}
 where $c$ is a constant. After some simplifications, we obtain
\begin{IEEEeqnarray}{LLL}
-x &+& \sqrt{x^2+y^2}=e^c := S, \\
y^2 &=& S^2+2Sx,
\label{ParS}
\end{IEEEeqnarray}
where $S$ is a parameter to be optimized (through HFSS simulations) to attain the best $S_{11}$ for the entire structure. The caps are fabricated using aluminum with a thickness of 5 mm. 

We have simulated two different scenarios to study the relative merits of optimized (curved) caps. Both scenarios targeted a center frequency of 5.8545 GHz. The objective was to improve TX antenna matching, i.e., reduce the $S_{11}$ of the TX antenna over the desired bandwidth centered at 5.8545 GHz. In the first scenario, two flat metallic caps were used to close the antenna structure's top and bottom. Tuning was performed on two parameters: 1) structure diameter; and 2) TX antenna length. These parameters were optimized (using HFSS simulations) while keeping all other parameters at their optimized values obtained beforehand. In the second scenario, caps with optimized curvature were used. Details of tuning are explained in Section~\ref{Tune}.
The conclusion was, to have a reasonable TX impedance matching, the diameter of the structure in the first scenario (flat caps) should be at least 7\% larger than the case of the second scenario. Nevertheless, for flat caps, the TX $S_{11}$ was rarely (for a small number of switching patterns) below -10 dB (see Fig.~\ref{fig:S11_flat}), while in the second scenario, it would  reach -20 dB for almost all switching patterns (see Fig.~\ref{tx_input_matching}, supported by measurement results shown in Fig.~\ref{tx_input_matchingm}). Table~\ref{TabIII} compares the radiation efficiency and maximum gain for the structure with flat caps (case 1) vs. the structure with curved caps (case 2). It is observed that the overall efficiency increases from 82\% (for flat caps) to 90\% (for curved caps). More importantly, the use of curved caps has guided the outgoing RF wave to concentrate around the horizontal plane - see improvement in maximum gain for case 2 vs. case 1 in Table~\ref{TabIII}, and the focused TX pattern in Fig.~\ref{TX-all}(c).
Finally, measurement results (see Fig.~\ref{tx_input_matchingm}) confirm that (using the curved caps) the $S_{11}$ parameter is acceptable for different switching patterns. 

\begin{comment} 
In the following study, we measured the ability of the antenna to focus the radiated power close to the horizontal plane. For this reason, two partial far-field spheres were defined in HFSS, one with an elevation range of ±20\degree and the other ±2\degree from the horizontal plane. In other words, in the first case, the far-field parameters were calculated on spherical coordinate when $\theta$ varies from 70\degree to 110\degree and $\phi$ varies from 0\degree to 360\degree, while in the second case $\theta$ varies from 88\degree to 92\degree and $\phi$ varies from 0\degree to 360\degree. The figures below show the antenna parameters calculated for the two mentioned cases at 5.8545\,GHz.

For different combinations of on and off walls, we observed that the radiated power is higher in the second scenario when the proposed caps are used. We can see that out of 1W, only about 820mW is radiated from the first structure while more than 900mW is radiated from the second structure. 
As Fig below shows, the maximum amount of radiated power intensity in the first scenario is about 186mW/sr and 145mW/sr for the first and second far-field surface cases, respectively, while we can see that when the proposed curved caps are used, this parameter increases to about 474mW/sr and 325mW/sr, for ±20\degree and ±2\degree beamwidths, respectively. This will prove that the radiation mostly takes place at the directions and beam-width which are quite desirable when we use the proposed caps.
\end{comment} 


\begin{table*}
\begin{center} 
\caption{Antenna radiation parameters at 5.8545\,GHz  for flat caps (case 1) and for caps with optimized curvatures (case 2). Maximum gain values are computed over a partial spherical far-field surface with $\theta$ deviating $\pm 20$\degree~from the horizontal plane. Accepted power accounts only for the impact of $S_{11}$. Radiated Power accounts for the impact of $S_{11}$ and the waste of energy in the antenna structure. Radiated Power is computed by integrating the energy flux density, i.e., the Poynting vector, over a sphere (at far-field) surrounding the entire antenna structure. Efficiency is defined as the ratio: Radiated Power/Incident Power.}
\begin{tabularx}{0.9\textwidth} { 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X  | }
  \hline
  Quantity & case 1 & case 2 \\
  \hline
   Incident Power & 1 W & 1 W \\
  \hline
    Accepted Power & 851.6 mW & 957.74 mW \\
  \hline
  Radiated Power & 820.9 mW  & 903.28 mW\\
  \hline
  Efficiency & 82.1\% & 90.3\% \\ \hline
    Peak Realized Gain & 2.35 & 5.96 \\
  \hline
\end{tabularx}
\label{TabIII}
\end{center}
\end{table*}

\begin{table*}
\begin{center}
\caption{Different walls' states selected for simulation of $S_{11}$ in Fig.~\ref{fig:S11_flat} and \ref{tx_input_matching}. Even though each of the three RF building blocks forming a wall can be switched independently, in Figs.~\ref{fig:S11_flat}, \ref{tx_input_matching} and \ref{tx_input_matchingm}, all switches on any of the walls ($1$ to $12$) have the same state (i.e., all three building block columns on a given wall are on for value 1, or all three are off for value 0).}
\begin{tabularx}{0.9\textwidth} { 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X  | }
  \hline
  State & SW1 & SW2 & SW3 & SW4 & SW5 & SW6 & SW7 & SW8 & SW9 & SW10 & SW11 & SW12\\ 
  \hline
  1 & 0 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 0 & 1 & 1 & 0\\ 
  \hline
  2	& 1	& 0	& 0	& 1	& 1	& 1	& 0	& 0 & 0 & 1 & 1 & 0 \\
  \hline
  3	& 1	& 1 & 1 & 0 & 0 & 1 & 1 & 0 & 1 & 1 & 1 & 0 \\
  \hline
  4	&1	&1	&1	&0	&0	&0	&1	&1	&1	&0	&0	&0 \\
  \hline
  5	&1	&0	&0	&0	&0	&1	&1	&0	&0	&1	&1	&1 \\
  \hline
  6	&1	&1	&1	&0	&0	&0	&0	&0	&0	&1	&1	&1 \\
  \hline
  7	&1	&0	&1	&0	&1	&0	&1	&0	&1	&1	&0	&1 \\
  \hline
\end{tabularx}
\label{Tabclw2}
\end{center}
\end{table*}


\begin{figure}[]
\centering
%\includegraphics[width=0.8\linewidth, trim={0, 0cm, 0, 1cm}]{./fig_rf/S11-sim}
\hspace{-0.5cm}\includegraphics[width=1\linewidth, trim={0, 0cm, 0, 1cm}]{./fig_rf/S11-sim.jpg}
\caption{$S_{11}$ of the TX antenna, with optimized caps, for 7 different walls' states mentioned in Table \ref{Tabclw2}  (HFSS simulation).}
\label{tx_input_matching}
\end{figure}


\begin{comment}
\begin{figure}[]
\begin{subfigure}{.5\textwidth}
  \centerline{\includegraphics[width=1\linewidth]{./fig_rf/Fig13_a.pdf}}
  \caption{}
\end{subfigure}%
\\
\begin{subfigure}{.5\textwidth}
   \centerline{\includegraphics[width=1\linewidth]{./fig_rf/Fig13_b.pdf}}
     \caption{}
\end{subfigure}
\caption{Control board PCB, (a) top layer, (b) bottom layer.}
\label{fig:control_board}
\end{figure}
\end{comment}
%
%\begin{figure}[t]
%\centerline{\includegraphics[width=1.\linewidth]{./fig_rf/S11-RX}}
%\caption{$S_{11}$ of the RX antenna (measurement result).}
%\label{fig:S11_RX}
%\end{figure}

\begin{figure*}[t]
\centerline{\includegraphics[width=1.\linewidth]{./fig_rf/S11-r.jpg}}
\caption{$S_{11}$ of the TX antenna (with optimized caps) for some configurations of on/off switches (measurement results).}
\label{tx_input_matchingm}
\end{figure*}

\subsection{Details of Surrounding Walls \label{sec:pcb_wall}}
The 12 side walls are made of RO4003C material with a thickness of 32 mil. On the outer face of each wall, the RX antenna and the PIN diodes control command signal traces are located. Part of the inside face of the wall is a large copper patch that acts as the RX patch antenna ground. The rest consists of three building block columns of small patches connected using SMP1320-040LF RF PIN diodes.
%As mentioned earlier, dimensions of patches are optimized such that by turning the PIN diodes on and off, the value of reflection coefficient (or the transmission coefficient) changes significantly. 
%For the initial estimation of the dimensions, we have considered that the wall consists of a building block which can be seen in Fig. \ref{fig:side_wall} with the two on and off states. The PIN diode is modeled as an ideal short or open circuit at this state. Also, we assumed that this building block will be repeated both in the x and y directions.  For this purpose, we defined Master/Slave boundary conditions both for the zx- and yz- planes.
%(Fig. \ref{fig:boundary_condition}). 
We defined two Floquet ports at the two sides of a boundary box to optimize the patch dimensions. Then, the reflection and the transmission coefficients, $S_{11}$ and $S_{21}$, respectively, are computed for different patch dimensions and also for the two states of on and off. Dimensions of the basic patch are optimized such that by turning the PIN diodes on and off, the value of the reflection coefficient (or the transmission coefficient) changes significantly. Relying on such an initial design, patch dimensions are then fine-tuned by simulating the entire antenna structure using HFSS. 

We randomly selected 7 different wall states to optimize the overall structure. These selected states are shown in Table~\ref{Tabclw2}. Fig.~\ref{tx_input_matching}  shows the TX antenna impedance matching, i.e., $S_{11}$ for these 7 states obtained through simulations.
The final patch size at 5.8545\,GHz is 5.6\,mm by 6\,mm wide. Furthermore, the width of the ground patch is around 37.5\,mm. There is a 1.6\,mm gap along the vertical axis between two adjacent patches in a building block column and a 1.5\,mm gap between two adjacent building block columns.  The radius of the structure where the PCBs are located is around 119\,mm from the center axis (z-axis). 
%In the following figures, Sw represents the building block states where 1 represents the on state, and 0 represents the off state.
%In the HFSS simulation, for each PIN diode, three boundary conditions are defined. 
% HERE 

The equivalent circuit for the PIN diode is composed of an inductance $L_s$ in series with a diode die equivalent circuit, where $L_s$ models the effect of the diode packaging. For SMP1320-040LF, we have\footnote{www.skyworksinc.com/-/media/SkyWorks/Documents/Products/101-200/SMP1320\_Series\_200047S.pdf} $L_s=0.45$\,nH.
The diode die itself is modeled by a parallel RC circuit in which values of the capacitor, $C_d$, and the resistor, $R_d$, depend on the diode state. Since $R_d$ in the on state (forward bias) is very small, i.e., $\simeq 0$, and in the off state (reverse bias) is very large,  i.e., $\simeq \infty$, it turns out that only the value of  $C_d$ in the off state affects the simulation outcome. Referring to MP1320-040LF application note$^{5}$, the value of $C_d$ in the off state (reverse bias capacitance) is set at $0.23$ pF. Although exact values of $R_d\simeq 0$ in the on (forward bias) and $R_d\simeq \infty$ in the off (reverse bias) sates do not affect the simulations outcomes, for the sake of completeness, here are the values we used in HFSS simulations: $R_d$(forward bias)\,=1\,Ohm and $R_d$ (reverse bias)\,=10\,MOhm.

\begin{comment}
We have used the following relations for the ON and OFF states:

\begin{IEEEeqnarray}{LLL}
\label{eq:eq_14}
C_d &=& S_w\times C_{on}+(1-S_w)\times C_{o\,f\,f}, \\
\label{eq:eq_15}
R_d &=& S_w\times R_{on}+(1-S_w)\times R_{o\,f\,f}.
\end{IEEEeqnarray}
where $S_w$ is the diode state. If it is in the on state, $S_w=1$, otherwise, $S_w=0$. In small-signal operation, the diode is modeled as a resistor in parallel with a capacitor. In forward bias, the small-signal resistance is very low and it decreases by increasing the bias current. When the diode is off, the resistance becomes much greater than the junction capacitance reactance and can be ignored. In simulations, this value is set at $R_{o\!f\!f}=10$\,MOhm.  
The modeled capacitor here is the junction capacitance, which also varies with the operating point. In simulation, we considered$^{5}$ that the reverse bias capacitance is 0.23 pF. In forward bias, the value of this capacitance increases, but since it is in parallel with a very small resistance, the exact value of forward capacitance does not have any noticeable impact on the simulation results. In simulations, this value is set at $C_{on}=10$\,pF.  
 
The values of the other constants are shown in Table~\ref{tab:resistance}. 
\begin{table}
\begin{center}
\caption{Values of resistance and capacitance in equations \eqref{eq:eq_14} and \eqref{eq:eq_15}.}
\label{tab:resistance}
\begin{tabularx}{0.48\textwidth} { 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X  | }
  \hline
  $C_{on}$ & $C_{o\!f\!f}$ & $R_{on}$ & $R_{o\!f\!f}$\\ 
  \hline
  10\,pF  & 0.23\,pF & 1\,Ohm & 10\,MOhm\\ 
  \hline
\end{tabularx}
\end{center}
\end{table}
\end{comment}

\subsection{Details of the RX Antenna}
The RX antenna is a planar patch element that is fed through a microstrip trace. On each wall, we have one RX antenna and a plane that acts as the patch antenna ground, i.e., the body of the antenna connector will be soldered to it. To have a higher bandwidth, the corners of the patch have been chamfered. Also, the inset feeding technique has been used for matching purposes (similar to the TX antenna).
Several parameters in the RX antenna were tuned at the desired center frequency of 5.8545\,GHz. These parameters include patch width, patch length, chamfer dimensions, inset length, and trace width. Fig.~\ref{fig:rx_antenna} shows the RX antenna, and Table~\ref{tab:rx_antenna_dimensions} shows final dimensions after fine-tuning in the presence of the entire antenna structure.
 Parameter $S_{11}$ for the RX antenna is shown in Fig.~\ref{fig:input_matching2}(a)
(HFSS simulation) and in Fig.~\ref{fig:input_matching2}(b) (measurement). It is observed that the frequency of the point with minimum $S_{11}$ in Fig.~\ref{fig:input_matching2}(a) is slightly different from that of Fig.~\ref{fig:input_matching2}(b). Despite this slight disagreement between simulation and measurement, the measured $S_{11}$ at the target frequency of 5.8545\,GHz is at an acceptable level (about -10 dB). In RF, such a small mismatch between simulation and measurement is quite common and can be corrected.  The mismatch can be due to fabrication error or the difference between the parameters of materials used in fabrication vs. what is modeled in HFSS.  Computational inaccuracies can be corrected by targeting a (proportionally) higher frequency in simulation.  Fig. \ref{RX-pattern} shows the pattern of the receive antenna.
\begin{figure}[]
\centering
%\includegraphics[width=0.95\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/Fig_XXXVII.jpg}
\includegraphics[width=0.8\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/a2.pdf}
\caption{RX antenna (refer to Table~\ref{tab:rx_antenna_dimensions} for values of optimized dimensions).}
\label{fig:rx_antenna}
\end{figure}
\begin{table*}[h]
\begin{center}
\caption{RX antenna dimensions reported in millimeters.}
\begin{tabularx}{0.9\textwidth} { 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X  | }
  \hline
  w0 & w1 & w2 & w3 & w4 & h1 & h2 & h3 & h4 & h5 & h6\\ 
  \hline
  0.5 & 0.75 & 1.5 & 6.5 & 10.5 & 3.3 & 7.3 & 11.3 & 12.05 & 16.8 & 21.55\\ 
  \hline
\end{tabularx}
\label{tab:rx_antenna_dimensions}
\end{center}
\end{table*}
\begin{figure}[]
 \hspace{-.4cm}  \centerline{\includegraphics[width=0.95\linewidth, trim={0, 0cm, 0, 0cm}]{./fig_rf/RX3.jpg}}
\caption{RX antenna input matching: (a) HFSS simulation and (b) measurement.}
\label{fig:input_matching2}
\end{figure}
%Table~\ref{tab:rx_antenna_dimensions} contains the dimensions of the RX antenna.
\begin{figure}[htbp]
    \centerline{\includegraphics[scale = 0.6]{./fig_rf/RX-pattern.jpg}}
	\caption{Pattern of a receive antenna in the presence of the entire antenna structure. }
	\label{RX-pattern}
\end{figure}

\subsection{Details of the TX Antenna}
Noting the circular symmetry of the structure, an omni-directional TX antenna is needed to operate at the center of the cylindrical structure. A good candidate for this purpose is a planar monopole antenna. Fig. \ref{fig:tx_antenna} shows the designed antenna. The antenna is printed on a 60-mil RO4003C Rogers substrate. The top and the bottom ground patches are connected using vias and soldered to the connector's body. To improve TX matching, the inset feeding technique has been used. The following parameters are tuned in optimizing TX matching: the length of ground patches, the notch dimensions in the bottom ground patch, the length and width of the narrow trace of the monopole, dimensions of the wider part of the monopole, and finally, the inset feed length. TX antenna tuning has been performed in the presence of caps and PCB walls for a center frequency of 5.8545\,GHz. 
Fig. \ref{fig:tx_antenna} shows the TX antenna and Table \ref{tab:tx_antenna_dimensions} shows final dimensions after fine-tuning in the presence of the rest of the antenna structure (refer to Section~\ref{Tune}). 
\begin{figure}[!h]
\begin{subfigure}{.3\textwidth}
  \hspace{1.7cm}\centerline{\includegraphics[width=1.1\linewidth]{./fig_rf/Fig30_aa.pdf}}
  \caption{}
\end{subfigure}%
\\
\begin{subfigure}{.3\textwidth}
  \hspace{1.5cm}\centerline{\includegraphics[width=0.91\linewidth]{./fig_rf/Fig30_bb.pdf}}
     \caption{}
\end{subfigure}
\caption{TX antenna: (a) front view and (b) back view.}
\label{fig:tx_antenna}
\end{figure}
\begin{table*}
\begin{center}
\caption{TX antenna dimensions (in mm).}
\begin{tabularx}{0.9\textwidth} { 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X  | }
  \hline
  w0 & w1 & w2 & w3 & w4 & w5 & h1 & h2 & h3 & h4 & h5 & w6 & w7 & w8 & h6 & h7 & h8\\ 
  \hline
  1.008 & 0.5 & 1.25 & 0.7 & 2.5 & 3 & 9 & 13 & 16 & 20 & 30 & 1.5 & 4 & 10 & 5 & 6.5 & 9\\ 
  \hline
\end{tabularx}
\label{tab:tx_antenna_dimensions}
\end{center}
\end{table*}

\subsection{Control Board}
For driving the PIN diodes, we have designed a control board that is attached to the upper cap from outside of the structure (see Fig.~\ref{fig:multi-pattern_structure}). 
%which are connected to the pin header through hole connectors embedded on both the control board and each wall.
We have used an AD828 dual, low-power Op-Amp to drive the PIN diodes. This Op-Amp has 130 MHz 3-dB bandwidth at a gain equal to 2 dB and 450 V/µs slew rate. Since we have thirteen PIN diodes in each building block column, considering the forward voltage of 0.85 V for each PIN diode, one needs around 11 V to turn on all the diodes. The selected Op-Amp is able to perform this task since it operates using a ±15 V power supply.

\subsection{Iterative Optimization of Design Components} \label{Tune}
RX antenna is initially designed as a standalone element and then tuned in the presence of the rest of the structure to optimize the corresponding $S_{11}$ parameter.   Similarly, the TX antenna is initially designed as a standalone element by optimizing the corresponding $S_{11}$ parameter while achieving an omni-directional pattern.  
The patch dimensions are initially designed using Floquet ports, where the reflection coefficient, $S_{11}$, and the transmission coefficient, $S_{12}$, of the building block are monitored to approach a reflecting surface (in the on state) and a transparent surface (in the off state).
Next, the above initial designs are integrated into the larger structure and the underlying four design decisions, namely geometries of: 1) RX antenna; 2) TX antenna; 3) surrounding walls; and 4) caps, including curvature, i.e., the parameter $S$ in \eqref{ParS} and the two radii in Fig. \ref{TX-all}(c)) are tuned in an iterative manner. Objectives have been realizing good $S_{11}$ for antennas, a TX radiation pattern concentrated around the horizontal plane, and realizing desirable $S_{11}$ and $S_{12}$ for the walls focusing on the 7 different test states mentioned in Table \ref{Tabclw2}.   


\subsection{Simulation vs. Measurement Results}
Fig. \ref{tx_input_matchingm} shows some measurement results, which closely match the simulation results in Fig. \ref{tx_input_matching}. Due to space limitations, only four cases of measurement results are shown. Several other cases have been tested, including some that were not considered in the initial design optimization. Measurement results show that, in all cases,  the achieved value of $S_{11}$ remains at an acceptable level, and is rather insensitive to the state of switches. 
